Computing Optimal Joint Chance Constrained Control Policies

We consider the problem of optimally controlling stochastic, Markovian systems subject to joint chance constraints over a finite-time horizon. For such problems, standard Dynamic Programming is inapplicable due to the time correlation of the joint chance constraints, which calls for non-Markovian, and possibly stochastic, policies. Hence, despite the popularity of this problem, solution approaches capable of providing provably-optimal and easy-to-compute policies are still missing. We fill this gap by augmenting the dynamics via a binary state, allowing us to characterize the optimal policies and develop a Dynamic Programming based solution method.

==> commands.tex <==
%============== General ================%
\newcommand{\reals}{\mathbb{R}}
\newcommand{\nonnegativeReals}{\mathbb{R}_{\geq 0}}
\newcommand{\positiveReals}{\mathbb{R}_{>0}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\Id}{\mathrm{Id}}
\renewcommand{\d}{\mathrm{d}}
\DeclareMathOperator*{\range}{Range}
\DeclareMathOperator*{\kernel}{Ker}
\newcommand{\ones}{\mathbbm{1}}
\newcommand{\zeros}{\mathds{O}}
\newcommand{\eye}{I}
\newcommand{\transpose}[1]{#1^\top}
\newcommand{\T}[1]{\transpose{#1}}
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\inv}[1]{\inverse{#1}}
\newcommand{\pseudoinverse}[1]{#1^\dagger}
\newcommand{\pinv}[1]{\pseudoinverse{#1}}
\newcommand{\sample}[2]{#1^{(#2)}}
\newcommand{\entry}[2]{#1_{#2}}

%============== Probabilities ================%
\newcommand{\Q}{\mathbb{Q}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\empiricalP}[1]{\widehat\P_{#1}}
\newcommand{\empiricalQ}[1]{\widehat\Q_{#1}}
\newcommand{\expectedValue}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\lebesgueMeasure}[1]{\mathcal{L}^{#1}}
\newcommand{\diracDelta}[1]{\delta_{#1}}
\newcommand{\support}[1]{\text{supp}(#1)}

%============== Functions ================%
\newcommand{\tensorProd}[2]{#1\times #2}
\newcommand{\proj}[1]{\pi_{#1}}
\newcommand{\indicator}[1]{\ones_{#1}}

%============== OT-related commands ================%
\newcommand{\setPlans}[2]{\Pi(#1,#2)}
\newcommand{\probSpace}[1]{\mathcal{P}(#1)}
\newcommand{\Pp}[2]{\mathcal{P}_{#1}(#2)}
\newcommand{\pushforward}[1]{{#1}_{\#}}
\newcommand{\transportCost}[3]{W^{#1}(#2,#3)}
\newcommand{\kl}[2]{\text{KL}(#1\Vert #2)}
\newcommand{\tv}[2]{\text{TV}(#1,#2)}
\newcommand{\ball}[3]{\mathbb{B}_{#1}^{#2}(#3)}

%============== Math operators ================%
\let\argmin\relax
\let\argmax\relax
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\esssup}{ess\,sup}
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\epi}{epi}
\DeclareMathOperator*{\lip}{lip}

%============== Comments ================%
\newcommand\margincomment[4]{{\color{#3}#1}\marginpar{\vspace{-0\baselineskip}\color{#3}\raggedright\scriptsize [#4]:#2}}
\newcommand{\nlmargin}[2]{\margincomment{#1}{#2}{red}{NL}}
\newcommand{\lamargin}[2]{\margincomment{#1}{#2}{blue}{LA}}
